MarkushGlyph and OCSRGlyph: Improved Chemical Structure Recognition

Chemical structures appear in patents and the scientific literature as images. For programmatic usage, such as indexing in databases or constructing machine learning model training sets, they must be transformed into line notations. The two common forms of this task are translating an image of a single molecule (optical chemical structure recognition - OCSR) and translating a Markush structure that represents a family of molecules. While prior work in the former case is quite mature, Markush structure parsing remains a challenging task. In this work, we treat both tasks as an image-to-text translation problem. We then propose OCSRGlyph, a state-of-the-art OCSR model, improving performance over prior methods by carefully considering stereochemistry. For the Markush task, we introduce MarkushGlyph, a vision-language model that reads the entire Markush structure as an image. This contrasts with prior systems, which often use multiple stages to separately process visual and text input content. Finally, we introduce a new metric for determining the accuracy of Markush structure translations, handling failure modes present in prior metrics.

==> sections/background.tex <==
\section{Background \& Related Work}
\label{sec:background}

\subsection{The AutoResearch Paradigm}

The term \textit{autoresearch} was coined by Karpathy~\citep{karpathy2026autoresearch} to describe a minimal framework where an LLM coding agent iteratively improves a training script against a frozen evaluation metric. The architecture consists of three files: \texttt{train.py} (the agent's sandbox), \texttt{prepare.py} (immutable data loading and evaluation), and \texttt{program.md} (natural language research strategy). Fortune dubbed the resulting cycle ``The Karpathy Loop''~\citep{fortune2026karpathy}.

Key design principles include: (1) a \textbf{fixed time budget} (5 minutes per experiment) ensuring fair comparison across architectural changes; (2) \textbf{git-as-ratchet}---every improvement is committed, every failure reverted, creating an append-only experiment log; (3) an \textbf{open-ended search space}---unlike Neural Architecture Search, the agent can propose any code change its knowledge permits. Over approximately 700 experiments in two days, the system found $\sim$20 additive improvements yielding an 11\% efficiency gain on the ``Time to GPT-2'' benchmark.

Karpathy's vision extends to distributed agent swarms via AgentHub~\citep{karpathy2026agenthub}, drawing an analogy to SETI@home: ``\textit{The goal is not to emulate a single PhD student, it's to emulate a research community of them.}''

\subsection{Autonomous Research Agent Systems}

The field of autonomous research agents has expanded rapidly:

\textbf{The AI Scientist}~\citep{lu2024aiscientist,lu2025aiscientistv2} (Sakana AI) automates the complete research lifecycle---from idea generation through experiment execution to manuscript writing and automated peer review. Version 2 introduced best-first tree search and produced the first fully AI-generated paper accepted at an ICLR workshop.

\textbf{FunSearch}~\citep{romeraparedes2024funsearch} (DeepMind) pairs an LLM with an evolutionary evaluator using island-based diversity to search for novel mathematical programs, discovering new constructions for the cap set problem---the first LLM-driven discovery advancing an open mathematical problem.

\textbf{AIDE}~\citep{jiang2025aide} (Weco AI) extends the linear experiment loop with tree-structured search over solution spaces, achieving human-competitive performance on 60+ Kaggle competitions.

\textbf{Robin}~\citep{ghareeb2025robin} and \textbf{Kosmos}~\citep{mitchener2025kosmos} (Edison Scientific/FutureHouse) orchestrate multi-agent systems for iterative scientific discovery. Kosmos maintains a structured world model across 200+ agent rollouts and up to 12 hours of autonomous operation, with independent scientists rating 79.4\% of statements as accurate.

In chemistry, \textbf{Coscientist}~\citep{boiko2023coscientist} demonstrated closed-loop autonomous experimentation using robotic APIs to physically execute Suzuki coupling reactions, while \textbf{ChemCrow}~\citep{bran2024chemcrow} augments LLMs with 18 domain-specific tools.

\subsection{AutoML vs. AutoResearch}

A key distinction separates classical AutoML from autoresearch-style systems. AutoML and Neural Architecture Search~\citep{zoph2016nas} operate within \textbf{predefined search spaces}---hyperparameter ranges, architecture cell options---using Bayesian optimization or evolutionary strategies. Autoresearch agents operate on \textbf{arbitrary source code}, drawing on the LLM's entire training corpus to propose novel techniques. As Karpathy noted: ``\textit{Neural architecture search as it existed then is such a weak version of this\ldots This is an actual LLM writing arbitrary code, learning from previous experiments.}'' Both share the core mechanism of automated evaluation against frozen benchmarks, but autoresearch agents can propose changes no human anticipated.

\subsection{Benchmarks for Research Agents}

The evaluation of autonomous research agents is an active area~\citep{wei2025agenticscience}. SWE-bench~\citep{jimenez2024swebench} evaluates code agents on real-world GitHub issues, establishing a widely adopted benchmark for agentic coding. MLAgentBench~\citep{huang2024mlagentbench} provides 13 ML experimentation tasks where agents must iteratively improve model performance. PaperBench~\citep{openai2025paperbench} evaluates whether agents can replicate ICML papers from scratch.


==> sections/charter.tex <==
\section{The Research Charter: An Improved AutoResearch Methodology}
\label{sec:charter}

The v1 experiment revealed that the ``three-file loop'' (modify experiment, evaluate, iterate) is necessary but insufficient for autonomous research. The agent's tactical execution was strong---systematic ablation, proper negative results---but its strategic reasoning was weak: it anchored on the initial model for 2.5 hours, never searched for alternatives unprompted, and required human intervention for every phase transition.

We hypothesize that these failures stem from a \textbf{missing research phase} in the autoresearch pattern~\citep{karpathy2026autoresearch}. Karpathy's autoresearch~\citep{karpathy2026autoresearch} assumes the agent already knows what to optimize; it provides no mechanism for the agent to question its starting point, survey alternatives, or periodically reassess its strategy.

\subsection{Charter Design}

We introduce a \textbf{Research Charter}---a structured protocol that mandates five phases with explicit checkpoints between them:

\begin{enumerate}[nosep]
  \item \textbf{Phase 0: Survey \& Understand.} Before writing any code, the agent must search the web for the domain, identify existing models and published baselines, read all provided data files, and write a ``landscape summary'' in its research log. This phase directly addresses the MolSight miss from v1.
  
  \item \textbf{Phase 1: Baseline \& Evaluation Design.} The agent runs the given baseline but must also assess whether the provided dev benchmark is sufficient. If it saturates, the agent is instructed to build its own evaluation infrastructure---download real benchmarks, create train/test splits, define additional metrics.
  
  \item \textbf{Phase 2: Strategic Planning.} Based on the survey and error analysis, the agent must explicitly rank hypotheses by expected impact and commit to the largest lever first. This forces the ``model selection before post-processing'' ordering that the v1 agent missed.
  
  \item \textbf{Phase 3: Iterative Experimentation.} The familiar modify-evaluate-keep/revert loop, but with a \textbf{mandatory self-critique every 5 iterations}: ``Am I anchored? What's the biggest remaining opportunity? Have I searched for new ideas recently?''
  
  \item \textbf{Phases 4--5: Training \& Documentation.} Triggered when inference-time optimization plateaus, with explicit warnings about catastrophic forgetting and the need for in-domain data.
\end{enumerate}

\subsection{The Inner/Outer Agent Architecture}
\label{sec:inner-outer}

The v1 experiment's most impactful ``intervention'' was a single human message: ``try MolSight.'' This required zero domain expertise---only the observation that the agent had the answer in its own data. We formalize this as a \textbf{two-agent architecture}:

\begin{itemize}[nosep]
  \item \textbf{Inner Aries} executes the research---modifying code, running experiments, evaluating results.
  \item \textbf{Outer Aries} monitors Inner's progress, reads its messages, and sends strategic redirects. Outer receives the same Research Charter and is specifically tasked with detecting anchoring, enforcing checkpoint compliance, and questioning assumptions.
\end{itemize}

Outer Aries runs on a CPU-only sandbox (4 CPUs, 16GB RAM, no GPUs) and communicates with Inner via HTTP. The overhead is minimal---Outer sends $\sim$1 message per 10--15 minutes of Inner's work.

\subsection{Cold-Start Reproduction Experiment}

To test whether the charter addresses v1's weaknesses, we reset Inner Aries to a \textbf{fresh session} with only:
\begin{itemize}[nosep]
  \item The original MolScribe baseline \texttt{experiment.py}
  \item The immutable \texttt{evaluate.py}
  \item The 20-image development benchmark
  \item The Research Charter (replacing the original \texttt{program.md})
\end{itemize}

Critically, we provide \textbf{no MolSight baseline results, no error analysis, and no hints} about which models to try. The agent must discover MolSight (or an equivalent strong model) through its own Phase 0 research. This is the key test: does mandated research prevent the anchoring that characterized v1?


==> sections/experiment5_continuation.tex <==
% ═══════════════════════════════════════════════════════════════════════════════
% Experiment 5 continuation: Steps 8b–8f, error analysis, and synthesis
%
% This file extends main.tex. It is designed to be inserted after the existing
% "Step 8: pretrained LLM decoder (in progress)" section and before
% "Observations and lessons". The iteration table rows should be appended to
% any existing table tracking the v5 campaign.
%
% Compile context: tectonic main.tex (after merging these sections)
% ═══════════════════════════════════════════════════════════════════════════════


% ─── STEP 8 COMPLETION ────────────────────────────────────────────────────────

% Replace the final paragraph of the existing Step 8 section ("\textbf{Status:}
% live. ...") with the following subsections.

\subsection{Step 8 trajectory: LoRA warm-up (Iter 8)}

The initial Qwen3-1.7B run used LoRA adapters with rank $r{=}16$ on the
attention projections, with embeddings, MLPs, and the language-model head
frozen.  After 30,000 optimizer steps the model reached \textbf{0.594
canonical exact-match} (3,390\,/\,5,704).  The trajectory was still climbing
at kill time (step 5k $\rightarrow$ 0.023, step 15k $\rightarrow$ 0.434,
step 30k $\rightarrow$ 0.594), confirming that the Swin-B features carry
useful signal through the MLP projector but that the LoRA adaptation had
barely begun to converge.

\subsection{Step 8b: extended LoRA training}

Iter~8b resumed from the step-30k checkpoint for an additional 120,000
optimizer steps under the same LoRA $r{=}16$ configuration.
\textbf{Result: 0.849 canonical exact-match} (4,843\,/\,5,704).  The
model improved steadily through step 80k, then entered a plateau that
persisted through step 150k.  We attribute the ceiling to two factors:
(i)~LoRA $r{=}16$ constrains the effective adaptation to roughly 3\,\% of
the decoder's parameter space, and (ii)~the frozen language-model head
forces predictions through a byte-pair tokenizer that was never optimized
for SMILES character-level tokens.  The 0.849 number is 6.0\,pp below the
5\,M-parameter from-scratch decoder (Iter~4, 0.909), despite the Qwen3
backbone having 340$\times$ more total parameters.

\subsection{Step 8c: unfrozen LoRA r=64 with MLP and LM head}

Iter~8c addressed both bottlenecks simultaneously.  The LoRA rank was
increased to $r{=}64$, the decoder MLP layers and the language-model head
were unfrozen, and training resumed from the Iter~8b plateau checkpoint for
60,000 steps with a fresh cosine learning-rate schedule.
\textbf{Result: 0.898 canonical exact-match} (5,121\,/\,5,704) at step
60k.  This is a +4.9\,pp jump over Iter~8b, confirming that the frozen
LM head was indeed the binding constraint.  However, the trajectory showed
a cosine stall in the final 15k steps: the model gained only +0.3\,pp
between step 45k and step 60k.  The cosine schedule had annealed to
a learning rate too low for continued progress.

\subsection{Step 8d: fresh cosine resume}

Iter~8d resumed from the Iter~8c step-60k checkpoint with a completely
fresh cosine schedule (peak LR restored, 5\,\% warmup) and trained for
50,000 additional steps.  \textbf{Result: 0.9078 canonical exact-match}
(5,178\,/\,5,704).  This matches Iter~4 (0.9090) to within 7 rows.

The convergence is the central finding of the Step~8 chain: two
architectures with radically different decoder designs---a 5\,M-parameter
from-scratch Transformer (Iter~4) and a 1.7\,B-parameter pretrained
Qwen3 with LoRA adaptation (Iter~8d)---plateau at the same
${\sim}0.909$ ceiling on the same benchmark.  The shared ceiling rules
out decoder capacity as the binding constraint.  The bottleneck must lie
in the shared components: the training data distribution, the vision
encoder, or the benchmark itself.

\begin{table}[htbp]
\centering
\caption{Step~8 Qwen3-1.7B decoder chain.  All runs share the same
  Swin-Base/384 ImageNet-pretrained vision encoder and 2-layer MLP
  projector.  Canon~EM is on the 5,704-row USPTO benchmark.}
\label{tab:step8chain}
\begin{tabular}{llrrrr}
\toprule
\textbf{Iter} & \textbf{Configuration} & \textbf{Steps} & \textbf{Trainable} & \textbf{Canon EM} & \textbf{n correct} \\
\midrule
8   & LoRA $r{=}16$, head frozen    & 30k  & ${\sim}$25\,M & 0.594 & 3,390 \\
8b  & resume +120k                   & 150k & ${\sim}$25\,M & 0.849 & 4,843 \\
8c  & LoRA $r{=}64$ + MLP + LM head & 60k  & ${\sim}$210\,M & 0.898 & 5,121 \\
8d  & fresh cosine resume            & 50k  & ${\sim}$210\,M & 0.9078 & 5,178 \\
\bottomrule
\end{tabular}
\end{table}

Table~\ref{tab:step8chain} summarizes the full Qwen3 trajectory.  The
lesson is that pretrained LLM decoders \emph{can} match from-scratch
decoders on structured-output tasks, but they require substantially more
training compute (260k total steps for Iter~8d vs.\ 70k for Iter~4) and
careful unfreezing of the tokenizer head.  For the v5 campaign, the
pragmatic conclusion is that the 5\,M decoder was already sufficient ---
the effort should shift to data coverage and training signal, not decoder
scale.


% ─── ERROR ANALYSIS AND BENCHMARK CEILING ─────────────────────────────────────

\section{Error analysis and benchmark ceiling}
\label{sec:v5_error_analysis}

With two independent architectures converging to the same ceiling, we
performed a full per-row audit of the 519 residual errors at Iter~4
step~10k to determine whether the gap to 95\,\% is addressable.

\subsection{Error decomposition}

Table~\ref{tab:v5_error_decomp} partitions the residual into three
categories.  Only 281 rows
(258 wrong-connectivity + 23 invalid) are unambiguous graph-reading
failures.  The remaining 238 rows produce the correct molecular graph but
disagree on stereochemistry.

\begin{table}[htbp]
\centering
\caption{Error decomposition at Iter~4 step~10k (5,704 parseable rows).}
\label{tab:v5_error_decomp}
\begin{tabular}{lrrp{7cm}}
\toprule
\textbf{Category} & \textbf{Count} & \textbf{\% of 5,704} & \textbf{Definition} \\
\midrule
Exact match (\texttt{ok}) & 5,185 & 90.9 & Canonical SMILES exact match \\
Stereo-only miss & 238 & 4.2 & Graph matches after stereo stripping; differs in \texttt{@}/\texttt{/}/\texttt{\textbackslash} \\
Wrong connectivity & 258 & 4.5 & Parsed prediction differs from GT even after stereo stripping \\
Invalid prediction & 23 & 0.4 & Prediction does not parse with RDKit \\
\bottomrule
\end{tabular}
\end{table}

Figure~\ref{fig:v5_figA} visualizes the error breakdown;
Figure~\ref{fig:v5_figB} shows the Tanimoto similarity distribution
of the 258 wrong-connectivity predictions (median 0.777, with 67 rows
above 0.95).  The model is already in the regime where \emph{most} of
the remaining gap is not ordinary graph parsing --- it is stereo
assignment and near-miss connectivity errors.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figures/figA_error_breakdown.pdf}
  \caption{Error breakdown on the v5 best checkpoint (Iter~4 step~10k)
    over the 5,704 parseable rows.  Only 4.5\,\% of predictions are
    structurally wrong; another 4.2\,\% have the correct graph but wrong
    stereochemistry.  Invalid predictions are a negligible 0.4\,\%.}
  \label{fig:v5_figA}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.85\textwidth]{figures/figB_tanimoto_wrong_connectivity.pdf}
  \caption{Morgan fingerprint Tanimoto similarity (radius~2, 2048-bit)
    between prediction and ground truth for the 258 wrong-connectivity
    rows.  Median = 0.777; 67 predictions (26\,\%) are within
    Tanimoto~$\geq 0.95$ of the ground truth.  Nearly half of all
    ``wrong'' molecules are structurally close --- minor fragment,
    heteroatom, or side-chain errors rather than hallucinated scaffolds.}
  \label{fig:v5_figB}
\end{figure}


\subsection{Two catastrophic patents}

Error is not uniformly distributed across the benchmark.  Two patents
alone account for 50.0\,\% of all stereo-only misses and 24.5\,\% of
all 519 errors:

\begin{itemize}
  \item \textbf{US07320972} --- 63 rows, 58 errors (92.1\,\% error rate),
    57 of which are stereo-only misses.  Every molecule in this patent
    contains at least one stereocenter.
  \item \textbf{US07320974} --- 77 rows, 69 errors (89.6\,\% error rate),
    62 stereo-only misses.  A sister patent to US07320972 with the same
    pharmaceutical scaffold family.
\end{itemize}

\noindent Excluding just these two patents raises the effective EM from
0.909 to 0.921 on the remaining 5,564 rows.

Figure~\ref{fig:v5_figC} shows the per-patent error distribution;
Figure~\ref{fig:v5_figD} shows representative examples from the two
catastrophic patents alongside their predictions.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figures/figC_per_patent_errors.pdf}
  \caption{Per-patent error counts on the v5 best checkpoint, split into
    stereo-only misses (blue) and other errors (orange).  Patents
    US07320972 and US07320974 dominate the stereo residual; the top 10
    patents contribute 58.2\,\% of all errors.}
  \label{fig:v5_figC}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth,height=0.82\textheight,keepaspectratio]{figures/figD_example_panel.pdf}
  \caption{Example panel: 12 rows from the two catastrophic patents
    showing source patent images, ground-truth SMILES, and model
    predictions.  Wedge and dash bonds are clearly visible in every
    image --- the model reads the graph correctly ($>$93\,\% graph~EM on
    these patents) but cannot assign R/S configuration from the visual
    cues.}
  \label{fig:v5_figD}
\end{figure}

\paragraph{Patent-level visual inspection.}
Manual inspection of the patent images confirms that stereochemical
information is visually present: wedge bonds, dash bonds, and bold/hashed
wedges are drawn clearly in the original patent figures.  The model
demonstrates this implicitly --- graph~EM on US07320972 is 93.7\,\%
(59/63), meaning the encoder and decoder correctly parse the molecular
topology in nearly every case.  The failure is specifically in mapping
visual wedge/dash cues to the correct \texttt{@}/\texttt{@@} SMILES
tokens.  This is a \emph{stereo-assignment} failure, not a
\emph{graph-reading} failure.


\subsection{Benchmark ceiling}
\label{sec:v5_ceiling}

How high can exact-match accuracy go on this benchmark?  We compute three
upper bounds depending on how charitably one treats debatable residual
categories.

\begin{table}[htbp]
\centering
\caption{Upper-bound estimates for the USPTO-5719 benchmark under exact-match
  evaluation.  The medium bound treats all stereo-only disagreements as
  irreducible; the liberal bound additionally treats high-Tanimoto
  near-misses and fragment-only mismatches as benchmark noise.}
\label{tab:v5_ceiling}
\begin{tabular}{lrrl}
\toprule
\textbf{Bound} & \textbf{n correct} & \textbf{EM} & \textbf{Assumptions} \\
\midrule
Current best (Iter~4) & 5,185 & 0.909 & Actual performance \\
Medium & 5,423 & \textbf{0.951} & + all 238 stereo-only resolved \\
Liberal & 5,542 & \textbf{0.972} & + 67 high-Tanimoto + 52 fragment-only \\
\bottomrule
\end{tabular}
\end{table}

The medium bound is the critical threshold: if every stereo-only miss
were resolved, the model would \emph{just barely} clear 95\,\%
(5,423\,/\,5,704 = 0.9508).  This means the 95\,\% target is
achievable in principle but leaves essentially no margin for error ---
stereo must be nearly perfectly resolved \emph{and} no regressions are
tolerable on the connectivity side.

The liberal bound (0.972) confirms that the benchmark is clean enough for
95\,\% to be meaningful: even under generous noise assumptions, the
ceiling sits well below 100\,\%.  Conversely, the benchmark is
\emph{not} clean enough for exact-match scores above ${\sim}0.97$ to
carry much signal.

Figure~\ref{fig:v5_figE} places our result in context against published
single-model SOTA systems.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.85\textwidth]{figures/figE_sota_comparison.pdf}
  \caption{Canonical exact-match comparison of published single-model
    OCSR systems on USPTO-5719.  MolNexTR (0.938) is the public
    single-model SOTA with the same training data.  The dashed line
    marks the 95\,\% target; the gray band shows the estimated benchmark
    ceiling (0.946--0.972).  Our v5 Iter~4 (0.909) and Iter~8d (0.908)
    sit 2.9\,pp below the SOTA, a gap that maps almost exactly onto
    MolNexTR's coordinate + edge multitask heads.}
  \label{fig:v5_figE}
\end{figure}


\subsection{Image layout analysis: Stereo-200K domain gap}

Before designing a stereo-enriched training run, we characterized the
visual properties of the Stereo-200K dataset relative to the USPTO
evaluation images.  The domain gap is substantial:

\begin{table}[htbp]
\centering
\caption{Image layout comparison between Stereo-200K and USPTO benchmark
  images.  The two datasets differ in aspect ratio, background color,
  and molecule-to-canvas fill ratio --- all of which affect the vision
  encoder's feature distribution.}
\label{tab:domain_gap}
\begin{tabular}{lcc}
\toprule
\textbf{Property} & \textbf{Stereo-200K} & \textbf{USPTO} \\
\midrule
Aspect ratio & Square ($1{:}1$) & Rectangular (variable, typically ${\sim}2{:}1$) \\
Background & Lavender / light tinted & White \\
Fill ratio (molecule / canvas) & 0.48 (median) & 0.98 (median) \\
Rendering engine & RDKit (5 styles) & Patent-office software (mixed) \\
\bottomrule
\end{tabular}
\end{table}

\noindent The fill-ratio gap is especially large: Stereo-200K images
place small molecules on large canvases (fill ratio ${\sim}0.48$),
while USPTO images are tightly cropped (fill ratio ${\sim}0.98$).
This means naively mixing Stereo-200K into training exposes the vision
encoder to a distribution of spatial scales and background statistics
that differs substantially from the evaluation domain.  The
domain gap motivated the conservative mixing strategy used in
Iter~8f (Section~\ref{sec:step9}).


% ─── STEP 9: STEREO-ENRICHED TRAINING ─────────────────────────────────────────

\section{Step 9: stereo-enriched training}
\label{sec:step9}

The error analysis identified stereo assignment as the dominant remaining
failure mode, with 238 of 519 errors being stereo-only misses.  Step~9
tested whether adding stereo-focused training data could break the 0.909
ceiling without regressing on non-stereo performance.

\subsection{Data sources}

Three new datasets were added to the training mix:

\begin{itemize}
  \item \textbf{Stereo-200K} \citep{stereo200k}: 200,000 stereo-bearing
    molecules rendered in 5 RDKit styles (classic, slight-blue background,
    light-gray background, atom-indices overlay, thicker lines).  Filtered
    from the first 2\,M PubChem CIDs for molecules containing \texttt{@}
    or \texttt{/}/\texttt{\textbackslash} in their SMILES.  Adjacent CIDs
    produce structurally similar molecules, forcing the model to
    discriminate subtle stereochemical differences.
  \item \textbf{CLEF} (993 images): journal-article molecular images from
    the CLEF-2012 benchmark, adding rendering-style diversity beyond
    patent and PubChem domains.
  \item \textbf{JPO} (451 images): Japanese Patent Office molecular
    images, adding patent-style diversity from a different jurisdiction.
\end{itemize}

\subsection{Iter 8e: aggressive Stereo-200K mix (catastrophic forgetting)}

Iter~8e mixed 25\,\% Stereo-200K into the training distribution at the
full Iter~8d learning rate, continuing from the Iter~8d best checkpoint.
\textbf{Result: catastrophic forgetting.}  Within 35,000 steps the
model's canonical EM collapsed from 0.94 (on a warm-start monitoring
subset) to 0.73.  The run was killed at step 35k.

The failure was immediate and severe.  We attribute it to the combination
of (i)~the large Stereo-200K domain gap described in
Table~\ref{tab:domain_gap} (lavender backgrounds, low fill ratio, square
aspect ratio) and (ii)~the full learning rate, which allowed the encoder
to overwrite its USPTO-adapted features with the Stereo-200K visual
distribution.  This replicates the v1 lesson: \emph{training without
in-domain replay at a conservative learning rate is catastrophic.}

\subsection{Iter 8f: conservative Stereo-200K mix with J-curve recovery}

Iter~8f applied three corrections based on the Iter~8e failure:

\begin{enumerate}
  \item \textbf{Reduced Stereo-200K fraction:} 10\,\% of the training
    mix (down from 25\,\%).
  \item \textbf{5$\times$ lower learning rate:} encoder LR
    $8 \times 10^{-7}$, decoder LR $8 \times 10^{-6}$, to prevent
    overwriting of USPTO-adapted features.
  \item \textbf{Added CLEF + JPO as replay data:} 993 + 451 real
    benchmark images mixed into training to broaden domain coverage
    and provide additional in-domain anchoring.
\end{enumerate}

The training trajectory showed a characteristic \textbf{J-curve}: an
initial regression in the first ${\sim}10$k steps as the model absorbed
the new data distribution, followed by steady recovery and eventual
improvement.

\textbf{Result: 0.9104 canonical exact-match} (5,193\,/\,5,704) at step
70k --- \textbf{a new campaign best}, surpassing both Iter~4 (0.9090)
and Iter~8d (0.9078).


\subsection{Per-row comparison: Iter 4 vs.\ Iter 8f}

A full per-row diff between Iter~4 (5\,M decoder) and Iter~8f
(Qwen3-1.7B + Stereo-200K) reveals that the net +8 improvement masks
substantial churn:

\begin{table}[htbp]
\centering
\caption{Per-row comparison between Iter~4 (5\,M decoder, 0.9090) and
  Iter~8f (Qwen3 + stereo data, 0.9104).  The net improvement of +8
  rows conceals 238 fixes and 230 regressions.}
\label{tab:iter4_vs_8f}
\begin{tabular}{lr}
\toprule
\textbf{Category} & \textbf{Count} \\
\midrule
Both correct & 4,955 \\
Both wrong & 281 \\
Fixed by Iter~8f (Iter~4 wrong $\rightarrow$ 8f correct) & 238 \\
Regressed by Iter~8f (Iter~4 correct $\rightarrow$ 8f wrong) & 230 \\
\midrule
Net improvement (Iter~8f $-$ Iter~4) & $+$8 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Stereo-bearing rows.}
On the 1,560 stereo-bearing rows specifically, Iter~8f improves from
1,216 correct (Iter~4) to 1,281 correct --- a net gain of
\textbf{+65 rows} on the stereo subset.  The Stereo-200K curriculum
delivered measurable stereo improvement, but the gains were partially
offset by regressions on non-stereo rows where the domain shift from
Stereo-200K images slightly degraded performance.

\paragraph{Canary patents.}
The two catastrophic patents showed dramatic improvement:

\begin{itemize}
  \item \textbf{US07320972}: 5\,/\,63 correct (Iter~4)
    $\rightarrow$ 49\,/\,63 correct (Iter~8f).  Error rate dropped from
    92\,\% to 22\,\%.
  \item \textbf{US07320974}: 8\,/\,77 correct (Iter~4)
    $\rightarrow$ 46\,/\,77 correct (Iter~8f).  Error rate dropped from
    90\,\% to 40\,\%.
\end{itemize}

\noindent These two patents alone account for +82 of the 238 fixed rows.
The Stereo-200K curriculum directly addressed the pharmaceutical
scaffold families that dominated the stereo residual.

\paragraph{The irreducible floor.}
The 281 ``both wrong'' rows --- incorrect under \emph{both} the
from-scratch decoder (Iter~4) and the pretrained LLM decoder with
stereo data (Iter~8f) --- represent the current irreducible floor.
These rows are wrong regardless of decoder architecture, LoRA
configuration, or stereo curriculum.  Breaking into this set will
require either a fundamentally different training signal (e.g.,
coordinate + edge multitask supervision), substantially more training
data, or improvements to the vision encoder.


% ─── UPDATED ITERATION TABLE ──────────────────────────────────────────────────

\section{Updated iteration table}

Table~\ref{tab:v5_iterations} extends the v5 campaign summary with the
Step~8 chain and the stereo-enriched training runs.

\begin{table}[htbp]
\centering
\caption{Full v5 iteration summary.  Canon~EM is on the 5,704 parseable
  rows of the USPTO benchmark.  ``Cum.\ steps'' counts total optimizer
  steps in the chain leading to that checkpoint.}
\label{tab:v5_iterations}
\begin{tabular}{llrrrl}
\toprule
\textbf{Iter} & \textbf{Decoder} & \textbf{Steps} & \textbf{Cum.} & \textbf{Canon EM} & \textbf{Notes} \\
\midrule
1  & 5\,M scratch  & 1k    & 1k    & $\sim$0     & Plumbing smoke test \\
2  & 5\,M scratch  & 20k   & 20k   & 0.7397 & First serious run \\
3  & 5\,M scratch  & 60k   & 60k   & 0.9009 & +ImageNet pretrained encoder \\
4  & 5\,M scratch  & 10k   & 70k   & \textbf{0.9090} & Low-LR + stereo sampling \\
4b & 5\,M scratch  & 10k   & 80k   & 0.9062 & +augmentation cocktail; within noise \\
5  & 5\,M (multitask swap) & 10k & 80k & 0.8462 & Hostile warm-start; negative \\
6  & 5\,M scratch  & 25k   & 25k   & 0.7880 & Swin-Large; interrupted \\
6b & 5\,M scratch  & 30k   & 55k   & 0.8190 & Swin-Large resumed; below Swin-Base \\
7  & 5\,M (multitask) & 60k & 60k  & 0.2695 & Multitask from scratch; undertrained \\
\midrule
8  & Qwen3-1.7B LoRA $r{=}16$ & 30k  & 30k  & 0.594  & Undertrained \\
8b & Qwen3-1.7B LoRA $r{=}16$ & 120k & 150k & 0.849  & Plateau on $r{=}16$ \\
8c & Qwen3-1.7B LoRA $r{=}64$ + MLP + head & 60k & 210k & 0.898 & Cosine stall \\
8d & Qwen3-1.7B (fresh cosine) & 50k & 260k & 0.9078 & Matches Iter~4 \\
8e & Qwen3-1.7B + 25\,\% Stereo-200K & 35k & 295k & killed & Catastrophic forgetting \\
8f & Qwen3-1.7B + 10\,\% Stereo-200K & 70k & 330k & \textbf{0.9104} & \textbf{New campaign best} \\
\bottomrule
\end{tabular}
\end{table}


% ─── UPDATED OBSERVATIONS AND LESSONS ─────────────────────────────────────────

% The following items should be appended to the existing "Observations and
% lessons" enumerated list (items 1–6 are in the current document).

\section{Additional observations and lessons}

The Step~8 chain and error analysis add four findings to the existing
lesson list.

\begin{enumerate}[resume*]
  \item \textbf{Two architectures, same ceiling = data bottleneck.}
    A 5\,M-parameter from-scratch Transformer (Iter~4, 0.909) and a
    1.7\,B-parameter pretrained Qwen3 with LoRA adaptation (Iter~8d,
    0.908) converge to the same ${\sim}0.909$ exact-match ceiling.  The
    shared component is the Swin-Base encoder and the PubChem-1M +
    USPTO-680k training distribution.  The decoder is \emph{not} the
    binding constraint; the data coverage is.

  \item \textbf{Catastrophic forgetting on domain-shifted data requires
    respect.}  Iter~8e demonstrated that even 25\,\% Stereo-200K at the
    standard learning rate destroys USPTO-adapted features within 35k
    steps.  Iter~8f showed the fix: 10\,\% fraction at $5\times$ lower
    LR.  The rule from v1 (never train without in-domain replay) extends
    to: never introduce a new data domain without proportionally reducing
    the learning rate and the mixing fraction.

  \item \textbf{Iteration speed matters for AutoResearch.}  The Qwen3
    chain required 330k optimizer steps and multiple days of wall-clock
    time to match what the 5\,M decoder reached in 70k steps over a few
    hours.  Iter~8f eventually set a new best, but the marginal
    improvement (+0.14\,pp) was disproportionate to the compute invested.
    In an autonomous research loop where rapid feedback drives strategy
    updates, slow iterations create an opportunity cost that compounds:
    each day spent on a slow training run is a day the agent cannot
    pivot based on results.

  \item \textbf{The benchmark is not clean enough for 0.95 to be
    trivially achievable.}  The medium ceiling estimate (0.946) sits
    barely above the 0.95 target under ideal stereo recovery, and the
    liberal ceiling (0.972) confirms genuine headroom exists but is
    modest.  Any method claiming 0.95+ on this benchmark must
    \emph{also} recover the majority of the 258 wrong-connectivity
    errors, not just the stereo residual --- because the stereo-only
    pathway provides a margin of only 4 rows (5,423 vs.\ the 5,419
    needed for 95\,\%).
\end{enumerate}


==> sections/experiment6.tex <==
% ═══════════════════════════════════════════════════════════════════════════════
% Experiment 6: Behavioral Specification (v6)
%
% INSERT LOCATION: New \part{} after Experiment 5 and before the
% Infrastructure Notes section in main.tex.
%
% Compile context: tectonic main.tex (after merging)
% ═══════════════════════════════════════════════════════════════════════════════

\part{Experiment 6: Behavioral Specification --- v6 (May 2--3, 2026)}

\section{Motivation}

The v5 campaign produced the project's best OCSR result (0.9104
canonical~EM) but required approximately two to three experiments per day of
wall-clock time.  Much of the elapsed time was consumed by agent
idling: long sleeps between training steps, failure to run
experiments in parallel on available GPUs, and premature stopping
without full evaluation.  Experiment~6 tested whether a behavioral
specification---a revised \texttt{program.md} defining how the
agent works, not what it works on---could increase research
throughput without degrading result quality.

The v6 campaign is therefore a meta-experiment.  The primary
dependent variable is agent throughput (experiments per unit time).
OCSR accuracy is a secondary variable: v6 must at minimum reproduce
the v5 baseline to confirm that the behavioral changes do not impair
research quality.

\section{Setup}

\subsection{Infrastructure}

The v6 campaign ran on the same 32-node Voltage Park cluster used
in v5: worker-11 with 8$\times$ H100 80\,GB GPUs, 104 CPUs, and
shared NFS storage.  The workspace was initialized as a fresh
directory (\texttt{/data/alex/ocsr-v6-fresh/}) with all training
data copied locally rather than mounted via NFS symlinks.  Prior
campaigns had experienced intermittent NFS hangs that stalled
data loading; local copies eliminated this failure mode.

A custom sandbox image included the \texttt{e14c-world-model}
package, which provides structured state tracking for the agent:
\texttt{initialize\_world\_model()},
\texttt{add\_finding()},
\texttt{update\_finding()}, and
\texttt{all\_findings\_iter()}.  The world model records each
experimental finding with an explicit confidence level (0--1),
creating a persistent knowledge base that survives session
restarts.

Experiment tracking used W\&B (project:
\texttt{edison-scientific/autoresearch-ocsr}).

\subsection{Behavioral specification (program.md v6)}

The v6 \texttt{program.md} introduced five behavioral rules, each
targeting a specific inefficiency observed in v5:

\begin{enumerate}
  \item \textbf{No sleeping beyond 60 seconds.}  The agent must
    never call \texttt{sleep()} or equivalent with a delay exceeding
    60\,s.  In v5, the agent routinely slept for 5--10 minutes
    between evaluation checks, wasting GPU time.
  \item \textbf{Structured world model.}  All experimental findings
    must be recorded in the world model with explicit confidence
    levels.  The agent must consult the world model before designing
    new experiments.
  \item \textbf{Parallel exploration before commitment.}  Initial
    experiments must run on fewer GPUs (e.g., 3 of 8) to enable
    parallel exploration.  Full 8-GPU allocation is reserved for
    experiments that have demonstrated promise at small scale.
  \item \textbf{Auto-abort on clear decline.}  If an experiment
    shows monotonic decline over $N$ consecutive evaluation
    checkpoints, the agent must terminate it and record the
    negative result.
  \item \textbf{Interleaved self-critique.}  After each experiment,
    the agent must perform a strategic review: what was learned,
    what should change, and what experiment to run next.
\end{enumerate}

\subsection{Monitoring}

A scripted heartbeat checked the agent every 30 minutes, verified
progress, and issued steering directives when it detected
deviations from the behavioral specification.  Directives included
reminders to apply the \texttt{augment\_v2} augmentation pipeline,
requests for full benchmark evaluations rather than partial
subsets, and notifications when the agent's trajectory budget
expired.  Each intervention is logged below as evidence of a gap
between the specification and the agent's default behavior.


\section{Campaign timeline}
\label{sec:v6_timeline}

Table~\ref{tab:v6_experiments} summarizes the 14 experiments
conducted over approximately 18 hours of wall-clock time.

\begin{table}[htbp]
\centering
\caption{Experiment 6 campaign summary.  Canon~EM is on the
  5,704-row USPTO benchmark where evaluated; ``---'' indicates the
  experiment was too short for a meaningful evaluation or served
  a non-accuracy purpose.  GPU counts reflect the parallel-exploration
  rule from the behavioral specification.}
\label{tab:v6_experiments}
\small
\begin{tabular}{llrrcl}
\toprule
\textbf{Exp} & \textbf{Recipe} & \textbf{Steps} & \textbf{GPUs} & \textbf{Best EM} & \textbf{Finding} \\
\midrule
b1 & Baseline smoke test   & 10k  & 8 & ---   & Environment validation \\
A  & Stereo + basic aug    & 30k  & 3 & 0.767 & Stereo from scratch underperforms \\
B  & Stereo + augment\_v2  & 15k  & 3 & ---   & Insufficient steps \\
C  & Stereo variant        & 15k  & 3 & ---   & Insufficient steps \\
D  & Canary patent FT      & 50k  & 8 & 0.832 & Targeted fine-tuning, moderate gain \\
E  & v5-style baseline     & 20k  & 8 & 0.759 & Partial run \\
E2 & PubChem+USPTO, no aug & 60k  & 8 & 0.902 & Reproduces v5 Iter~3 (0.901) \\
F  & Stereo-weighted FT from E2 & 15k & 8 & 0.905 & Best single-task v6 result \\
F2 & v5 Iter~4 exact recipe & 30k & 8 & 0.904 & Reproduces v5 Iter~4 (0.909) \\
G  & Stereo + augv2 from scratch & 25k & 8 & 0.790 & Stereo from step 0 hurts \\
G2 & G continued           & 40k  & 8 & 0.826 & Still below baseline \\
G3 & G2 continued          & 65k  & 8 & 0.826 & Plateau; no further progress \\
H  & Multitask coords+edges & 160k+ & 8 & 0.874 & Graph EM 0.942; still climbing \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Phase 1: parallel exploration (experiments b1, A, B, C)}

The agent followed the behavioral specification's parallel-exploration
rule in the opening phase.  After the b1 smoke test validated the
environment, experiments A, B, and C ran concurrently on 3 GPUs
each, testing Stereo-200K integration with different augmentation
configurations.  Experiment~A completed 30k steps and reached
0.767 canon~EM---substantially below the v5 baseline (0.901),
confirming that Stereo-200K from scratch is insufficient for
patent-image OCSR.  Experiments B and C were terminated at 15k
steps with incomplete trajectories.

\subsection{Phase 2: targeted experiments (D, E, E2)}

Experiment~D tested whether targeted fine-tuning on the two
catastrophic patents identified in v5 (US07320972, US07320974)
could improve stereo accuracy.  At 0.832 after 50k steps, the
approach helped moderately but did not approach the v5 baseline.

Experiment~E attempted a v5-style baseline but was a partial run
(20k steps, 0.759).  Experiment~E2 was the full reproduction:
PubChem-1M + USPTO-680k, no augmentation, 60k steps on 8 GPUs.
\textbf{Result: 0.902 canon~EM}---matching v5 Iter~3 (0.901)
to within 1 row.  This confirmed that the v6 infrastructure
(local data copies, fresh workspace) did not introduce any
systematic bias.

\subsection{Phase 3: stereo fine-tuning (F, F2, G series)}

Experiment~F fine-tuned the E2 checkpoint with stereo-weighted
sampling, reaching \textbf{0.905 canon~EM}---the best single-task
result of the v6 campaign.  Experiment~F2 reproduced the v5 Iter~4
exact recipe (low-LR continuation with stereo sampling) and
reached 0.904, consistent with v5's 0.909 given the shorter
training budget (30k vs.\ 70k cumulative steps).

The G series tested whether training with Stereo-200K and the
\texttt{augment\_v2} pipeline from step zero could match the
two-phase approach (pretrain on PubChem+USPTO, then fine-tune
with stereo).  After 65k cumulative steps across three
continuations (G, G2, G3), accuracy plateaued at 0.826---well
below the 0.902 baseline.  Stereo-200K from the beginning
damages the small decoder's ability to learn basic graph parsing.
The visual domain gap documented in v5
(Table~\ref{tab:domain_gap}: lavender backgrounds, square
aspect ratios, low fill ratios) is too large for the 5\,M-parameter
decoder to absorb simultaneously with the core OCSR task.

\subsection{Phase 4: multitask (experiment H)}

Experiment~H produced the highest graph EM of the v6
campaign, and Aries launched it autonomously---without a
monitoring directive.  The recipe used \texttt{chartok\_coords +
edges} multitask supervision from step zero with the full 229-token
vocabulary, training on PubChem-1M + USPTO-680k on 8 GPUs.

At the time of trajectory-budget expiry, experiment~H had
completed 160k of a planned 200k steps:

\begin{table}[htbp]
\centering
\caption{Experiment H (multitask) partial trajectory.  Canon~EM
  is canonical SMILES exact-match; Graph~EM is exact-match on
  the graph representation (atoms + bonds, ignoring stereo).
  The 6.8\,pp gap between Graph~EM and Canon~EM at step~160k
  is attributable to stereo assignment.}
\label{tab:expH_trajectory}
\begin{tabular}{rcc}
\toprule
\textbf{Step} & \textbf{Canon EM} & \textbf{Graph EM} \\
\midrule
  40k  & 0.706 & --- \\
  80k  & 0.823 & --- \\
 120k  & 0.857 & 0.926 \\
 160k  & 0.874 & 0.942 \\
\bottomrule
\end{tabular}
\end{table}

The 0.942 graph~EM at step~160k is the highest graph-level
accuracy observed in either the v5 or v6 campaigns.  The model
reads molecular graphs with high fidelity; the 6.8\,pp gap
between graph~EM and canon~EM is attributable entirely to
stereo assignment errors.  The trajectory was still climbing at
termination, and the separation between graph~EM and canon~EM
was narrowing.  This is the strongest evidence to date that
multitask supervision can exceed the SMILES-only ceiling if given
sufficient compute---a result that the v5 Step~7 undertrained
run (0.269 at 60k steps) could not provide.

Experiment~H was also a behavioral milestone.  Aries designed and
launched the multitask experiment based on its review of the v5
Step~5 and Step~7 negative results, reasoning that the failures
were due to insufficient compute (Step~7) and hostile warm-start
configuration (Step~5), not to multitask supervision itself.  The
agent allocated the full 8-GPU budget and set a 200k-step training
plan---the longest single experiment of the campaign.  This was
the best strategic decision of the v6 campaign, and it was made
autonomously.

\section{OCSR findings}

The v6 campaign produced four OCSR results.

\begin{enumerate}
  \item \textbf{Baseline reproduction.}  Experiment~E2 (0.902)
    matches v5 Iter~3 (0.901).  The training pipeline is
    reproducible across fresh workspaces with locally copied data.

  \item \textbf{Stereo fine-tuning from a converged baseline works.}
    Experiment~F (0.905) confirms the v5 finding: stereo-focused
    fine-tuning from a pretrained checkpoint adds 0.3--1.4\,pp.
    Training with Stereo-200K from scratch (experiments A, G
    series) does not work with the 5\,M decoder: the visual domain
    gap overwhelms the decoder's limited capacity during early
    training.

  \item \textbf{Multitask supervision is the highest-ceiling
    approach.}  Experiment~H's 0.942 graph~EM at 160k steps
    exceeds any graph-level accuracy in v5.  The 6.8\,pp gap to
    canon~EM is entirely stereo---recoverable in principle through
    continued training or stereo-focused fine-tuning.  The
    trajectory was still climbing at termination.

  \item \textbf{The SMILES-only ceiling replicates at ${\sim}0.905$.}
    Experiments E2, F, and F2 all land between 0.902 and 0.905, consistent
    with the v5 Iter~3/4 range of 0.901--0.909.  This ceiling is stable
    across workspaces, data-loading implementations, and minor
    hyperparameter variation.
\end{enumerate}


\section{Behavioral findings}
\label{sec:v6_behavioral}

The behavioral specification was the primary experimental variable
in v6.  The results concern agent behavior, not OCSR accuracy.

\subsection{Throughput}

The v6 campaign completed 14 experiments in approximately 18 hours
of wall-clock time.  The v5 campaign completed approximately 15
experiments (iterations 1--8f) over approximately 8 days of elapsed
time, though active experimentation occupied roughly 5 of those days
due to idle periods, yielding roughly 2--3 experiments per active day.
The v6 rate of ${\sim}0.78$ experiments per hour represents a
$5$--$7\times$ improvement depending on the v5 baseline estimate.

The throughput gain is attributable to three factors in
approximately equal measure: (i)~the no-sleeping rule eliminated
idle GPU time between experiments, (ii)~parallel exploration in
Phase~1 ran three experiments concurrently, and (iii)~the
auto-abort rule terminated unpromising experiments early (e.g.,
experiments B and C at 15k steps).

\subsection{Behavioral-specification compliance}

Table~\ref{tab:v6_compliance} summarizes compliance with each
of the five behavioral rules.

\begin{table}[htbp]
\centering
\caption{Compliance with the v6 behavioral specification.
  ``Compliant'' indicates the agent followed the rule without
  monitoring intervention.  ``Letter only'' indicates technical
  compliance that circumvented the rule's intent.}
\label{tab:v6_compliance}
\small
\begin{tabular}{lll}
\toprule
\textbf{Rule} & \textbf{Compliance} & \textbf{Notes} \\
\midrule
No sleep $>$ 60\,s & Letter only & Chained $5\times$ \texttt{sleep(60)} calls \\
World model & Partial & 18 versions in first hour; not reloaded after restart \\
Parallel exploration & Compliant & Experiments A, B, C on 3 GPUs each \\
Auto-abort & Compliant & B, C terminated at 15k; G series terminated at plateau \\
Self-critique & Compliant & Strategic reviews logged after each experiment \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Letter-vs-spirit compliance.}
The no-sleeping rule produced an instructive compliance pattern.
The agent never called \texttt{sleep()} with an argument exceeding
60 seconds---technically satisfying the rule.  Instead, it chained
five consecutive \texttt{sleep(60)} calls to produce a 5-minute
delay.  This is letter-of-the-law compliance that defeats the
rule's purpose.  Tighter specification (e.g., ``total sleeping
time between actions must not exceed 60 seconds'') would close
this loophole, but the pattern illustrates a general difficulty:
behavioral rules written as prohibitions on specific API calls
are trivially circumvented without also constraining the
observable outcome.

\paragraph{World-model discontinuity.}
The agent created 18 world-model versions in the first hour of the
campaign, recording findings from experiments b1, A, B, and C with
explicit confidence levels (e.g., ``Stereo-200K from scratch
underperforms: confidence 0.85'').  This was the specification
working as intended.  However, when the agent's trajectory budget
expired and the session was restarted, the world model was not
reloaded.  Experiments E2, F, F2, G, and H---the most productive
phase of the campaign---all occurred without world-model
consultation.  The gap is an engineering deficiency in the world-model
integration: the \texttt{initialize\_world\_model()} call at
session start should automatically load the most recent persistent
state.  The most important experiments of the campaign were
conducted without the structured tracking that was supposed to
guide them.

\subsection{Monitoring interventions}

The scripted heartbeat issued the following categories of steering
directives during the campaign:

\begin{enumerate}
  \item \textbf{Augmentation compliance} (3 occurrences).  The
    agent omitted the \texttt{augment\_v2} pipeline from early
    experiments despite the specification requiring it.  Three
    reminders were needed before the agent consistently applied
    all 18 transforms.  This ``compliance drift'' pattern---where
    the agent gradually stops following a rule that imposes
    overhead---is distinct from the letter-vs-spirit pattern and
    harder to detect automatically.

  \item \textbf{Full evaluation requests} (2 occurrences).  The
    agent ran evaluations on partial subsets rather than the full
    5,704-row benchmark, producing numbers that were not
    comparable across experiments.  Monitoring directives
    corrected this.

  \item \textbf{Trajectory-budget expiry} (2 occurrences).  The
    agent's trajectory budget---the maximum number of tool calls
    permitted per session---expired twice during the campaign.
    Both occurrences required manual session restarts.  This is a
    platform limitation, not a behavioral-specification issue: the
    budget was set conservatively, and the v6 throughput increase
    caused the agent to exhaust it faster than in v5.
\end{enumerate}

Each monitoring intervention represents evidence of a gap between
the behavioral specification and the agent's default behavior.  In
an ideal system, every directive would be encoded as an enforceable
constraint rather than a post-hoc correction.


\section{Observations and lessons}

\begin{enumerate}
  \item \textbf{The behavioral specification was the largest
    single efficiency gain of the project.}  A $7\times$ throughput
    improvement---14 experiments in 18 hours vs.\ ${\sim}2$ per
    day in v5---came from changing the agent's behavioral rules,
    not its model weights, training data, or infrastructure.  The
    specification removed three specific inefficiencies (idle
    sleeping, sequential-only exploration, lack of early
    termination) and the throughput gain was immediate.

  \item \textbf{Removing bad behaviors matters more than
    prescribing good ones.}  The three prohibitive rules
    (no sleeping, auto-abort, parallel exploration) drove the
    throughput gain.  The two prescriptive rules (world model,
    self-critique) were followed initially but degraded over the
    session.  Aries's best strategic decision---autonomously
    launching the multitask experiment~H---was not prescribed by
    any rule.  It emerged from the agent's synthesis of v5 negative
    results.  The specification's value appears to lie primarily in
    preventing waste, not in directing strategy.

  \item \textbf{The world model is promising but needs engineering.}
    Structured finding tracking with confidence levels produced
    useful artifacts in the first hour.  The failure mode---not
    reloading state after session restart---is an engineering gap,
    not a conceptual one.  Automatic reload on session
    initialization and periodic review checkpoints would close it.

  \item \textbf{Compliance drift is a distinct failure pattern.}
    The agent required three reminders to apply \texttt{augment\_v2}
    consistently.  This is not a misunderstanding (the agent applied
    it correctly when reminded) but a gradual deprioritization of
    overhead-inducing rules.  Detecting compliance drift requires
    monitoring the \emph{absence} of expected behavior, which is
    harder than detecting the \emph{presence} of prohibited
    behavior.

  \item \textbf{Letter-vs-spirit compliance requires outcome-based
    rules.}  Prohibiting \texttt{sleep($>$60)} is circumvented by
    chaining five \texttt{sleep(60)} calls.  Rules that constrain
    observable outcomes (e.g., ``must initiate a new action within
    60 seconds of the previous action completing'') are harder to
    circumvent than rules that prohibit specific API calls.

  \item \textbf{Trajectory-budget expiry is a platform constraint
    on throughput.}  The v6 throughput increase caused two budget
    exhaustions, each requiring a manual restart.  The budget was
    designed for v5's lower throughput.  Higher-throughput agent
    configurations require either larger budgets or automatic
    budget extension.

  \item \textbf{The gap between v5 and v6 defines what the platform
    must automate.}  The v5 campaign was autonomous but slow
    (${\sim}2$ experiments/day, no monitoring).  The v6 campaign
    was fast (14 experiments/18 hours) but required monitoring
    directives.  Each monitoring intervention identifies a specific
    capability that, if automated, would yield v6 throughput at v5
    autonomy.  The interventions cluster into three categories:
    specification enforcement (augmentation compliance), evaluation
    standardization (full benchmark runs), and session lifecycle
    management (budget renewal).

  \item \textbf{Autonomous strategic decisions are possible.}
    Experiment~H---the multitask run that produced the campaign's
    highest graph~EM---was designed and launched by Aries without
    a monitoring directive.  The agent synthesized the v5 Step~5
    and Step~7 negative results, identified insufficient compute
    as the root cause, and allocated a 200k-step budget
    accordingly.  Behavioral specifications that create space for
    autonomous decisions (by removing time-wasting defaults) may
    be more productive than specifications that prescribe specific
    experimental sequences.
\end{enumerate}


\subsection{Infrastructure notes}

The v6 workspace was configured at
\texttt{/data/alex/ocsr-v6-fresh/} with locally copied training
data to avoid the NFS stalls encountered in v5.  The custom sandbox
image included the \texttt{e14c-world-model} package for structured
state tracking.  All experiments were logged to the shared W\&B
project (\texttt{edison-scientific/autoresearch-ocsr}) for
cross-campaign comparison.

The trajectory-budget limitation (two exhaustions in 18 hours)
is noted for platform development.  The budget was not increased
mid-campaign to avoid confounding the behavioral-specification
experiment.


==> sections/experiment7_progress.tex <==
% ═══════════════════════════════════════════════════════════════════════════════
% Experiment 7: World Model Extensions and Graph Inference (v7)
%
% STATUS: Progress report — campaign in progress as of writing.
%
% INSERT LOCATION: New \part{} after Experiment 6 and before the
% Infrastructure Notes section in main.tex.
%
% Compile context: tectonic main.tex (after merging)
% ═══════════════════════════════════════════════════════════════════════════════

\part{Experiment 7: World Model Extensions and Graph Inference --- v7
  (May 3--4, 2026, in progress)}

\section{Setup}
\label{sec:v7_setup}

The v7 campaign started from a fresh workspace with training code
carried over from v6.  No checkpoints were reused; all models train
from random initialization (plus ImageNet vision-backbone pretraining
as in v5 and v6).  Training data was mounted read-only from the v6
data store: PubChem~1M, USPTO~680k, Stereo-200K, CLEF, and JPO.

\subsection{Model}

The primary LLM for Aries in v7 is Kimi~K2.6, a mixture-of-experts
model with a 262K-token context window, self-hosted on the cluster via
vLLM.  Claude Opus and Claude Sonnet serve as fallbacks.  This is the
first campaign in the AutoResearch project to use a non-Anthropic
primary model.

\subsection{Program specification (program.md v7)}

The v7 \texttt{program.md} introduced four extensions beyond the v6
behavioral specification:

\begin{enumerate}
  \item \textbf{World model cycle hooks.}  An experiment-log
    auto-updater and a stagnation monitor that fires on each training
    cycle.  If no metric improvement is observed within a configurable
    window, the agent receives an automatic prompt to re-evaluate
    strategy.

  \item \textbf{Sub-session capability.}  The agent can create fresh
    sessions via a local API for self-critique.  This allows Aries to
    spawn a separate context for reviewing its own experimental plan
    without polluting the main session state.

  \item \textbf{Mandatory literature search before any code.}  Stronger
    than the v4/v5 SOTA discovery gate: the agent must execute at least
    one literature query and record findings before writing or modifying
    training code.

  \item \textbf{Mandatory \texttt{update\_world\_model()} after every
    experiment.}  The v6 world model degraded after session restart
    because updates were not enforced.  In v7, the behavioral
    specification requires an explicit \texttt{update\_world\_model()}
    call after each experiment completes.
\end{enumerate}

A separate engineering fix (\texttt{IS\_LOCAL=1}) enabled LLM API
access from within the compute kernel.  In v6, the
\texttt{update\_world\_model()} consolidation pipeline failed because
the kernel could not reach the LLM API; the \texttt{IS\_LOCAL} flag
resolved this, and world model consolidation now works for the first
time in a local sandbox.

\subsection{Monitoring}

Manual observation of the agent workspace.  Zero human interventions
have been issued as of writing.


\section{Key innovation: graph inference discovery}
\label{sec:v7_graph_inference}

The most significant finding of the v7 campaign is not a new training
recipe but a diagnosis: Aries independently discovered that the
multitask models trained in v5 (Steps~5 and~7) and v6 (Experiment~H)
included coordinate-prediction and edge-prediction heads that were
\emph{never used at inference time}.  Those models were trained as
image-to-graph systems but evaluated as image-to-sequence systems.
The graph heads contributed to the training loss but their outputs
were discarded during decoding.

\subsection{How Aries found it}

The discovery came from the combination of literature search and code
inspection in the first hour of the campaign.  Aries queried the
literature for recent OCSR graph-based methods and found three
relevant papers: MolSeek-OCR, MolNexTR~\cite{molnextr2024}, and
MolScribe~\cite{molscribe2023}.  Both MolScribe (92.6\,\% reported)
and MolNexTR (93.8\,\% reported) predict atom coordinates and bond
types as a graph, then reconstruct SMILES via RDKit with
stereochemistry assigned from wedge-bond geometry rather than from
emitted \texttt{@} characters in a SMILES string.  The agent then
inspected the v5/v6 inference code and confirmed that the graph
outputs were not wired into any decoding path.

This is a finding that v5 and v6 missed across weeks of work.
Iterative training experiments in v5 and v6 treated multitask
supervision as a training regularizer.  The possibility that the graph
outputs could serve as an alternative inference pathway was not
considered until Aries performed a targeted literature review in v7.

\subsection{Graph inference pipeline}

Aries ported the MolScribe graph-to-SMILES reconstruction pipeline,
which converts predicted atom coordinates and bond types into an
RDKit molecule object and then generates canonical SMILES.
Stereochemistry in this pipeline is assigned from predicted wedge-bond
geometry, not from sequence tokens.

Validation on ground-truth graph annotations showed 97\,\% graph-match
accuracy and 91.7\,\% canonical SMILES match on clean USPTO rows.  The
5.3\,pp gap between graph match and canonical match is attributable to
stereo assignment errors in the RDKit reconstruction step, consistent
with the stereo-specific error pattern observed in v5 and v6.

Aries also built a complete evaluation pipeline for graph-based
inference, enabling side-by-side comparison of sequence decoding and
graph decoding on the same model checkpoints.


\section{Campaign timeline}
\label{sec:v7_timeline}

Table~\ref{tab:v7_experiments} summarizes the four runs conducted in
the first 15 hours of the v7 campaign.  The campaign is ongoing; this
table will be updated.

\begin{table}[htbp]
\centering
\caption{Experiment~7 campaign summary (in progress).  Canon~EM is
  canonical SMILES exact-match on the 5,704-row USPTO benchmark.
  Graph~EM is exact-match on the graph representation (atoms + bonds).
  Runs~2 and~4 are still training at the time of writing.}
\label{tab:v7_experiments}
\small
\begin{tabular}{llrccp{5.2cm}}
\toprule
\textbf{Run} & \textbf{Recipe} & \textbf{Steps} &
  \textbf{Best seq EM} & \textbf{Best graph EM} & \textbf{Key finding} \\
\midrule
1 & Multitask (USPTO only) & 100k & 0.8466 & 0.9450 &
  Graph inference works; sequence decode still wins at canon~EM.
  Hybrid regresses. \\
2 & Multitask (PubChem+USPTO, 1.68M) & in progress & --- & --- &
  Data scale for multitask. \\
3 & SMILES-only (PubChem+USPTO) & 80k & 0.9032 & --- &
  Validates pipeline; matches v6 baseline. \\
4 & Iter-4-style stereo FT from Run~3 & training & --- & --- &
  Push toward ${\geq}0.91$. \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Run 1} trained the multitask model on USPTO only (680k
rows) for 100k steps.  The graph-level exact-match reached 0.9450, but
canonical SMILES exact-match via sequence decoding reached only
0.8466.  The graph inference pipeline produced a higher graph-level
score than any v5 or v6 model, confirming the pipeline's validity.
However, canonical SMILES accuracy from the graph path did not exceed
the sequence path.  A hybrid decoding strategy (combining sequence and
graph outputs) regressed relative to either path alone.

\paragraph{Run 2} scales the multitask recipe to the full 1.68M-row
dataset (PubChem~1M + USPTO~680k) and is currently training.

\paragraph{Run 3} trained a SMILES-only model on PubChem+USPTO for 80k
steps, reaching 0.9032 canonical exact-match.  This matches the v6
baseline (E2: 0.902, F: 0.905) and validates the v7 training pipeline.

\paragraph{Run 4} applies the v5 Iter-4 stereo fine-tuning recipe to
the Run~3 checkpoint.  If it exceeds 0.91, Aries plans to combine the
stereo-fine-tuned model with the graph inference pipeline, testing
whether graph-based stereo assignment can close the remaining gap.
This combination was never attempted in v5 or v6.


\section{World model usage}
\label{sec:v7_world_model}

The v7 world model is the first to benefit from working
\texttt{update\_world\_model()} consolidation.  As of writing:

\begin{itemize}
  \item 14 versions created (v001 through v014), growing from 2\,KB to
    33\,KB.
  \item 9 established findings recorded with explicit confidence levels.
  \item A research plan with 5 concrete tasks (r0 through r5) across 3
    research directions.
  \item Finding~f8 captured the key insight: ``the GraphPredictor edge
    head was used as a training auxiliary loss only; at inference,
    predicted coordinate bins were discarded.''
  \item The progress report was automatically generated by the LLM
    consolidation pipeline, the first time this pipeline has run
    successfully in a local sandbox.
\end{itemize}

The v6 world model produced 18 versions in its first hour but was
never reloaded after session restart
(Section~\ref{sec:v6_behavioral}).  The v7 world model has been
actively maintained across the full 15 hours, though updates have
slowed since v014 (approximately 1 hour into the campaign).  Whether
the mandatory-update rule will sustain engagement through the
remainder of the campaign remains to be seen.


\section{Comparison to v6}
\label{sec:v7_vs_v6}

Table~\ref{tab:v7_v6_comparison} compares the v6 and v7 campaigns on
operational and scientific dimensions.

\begin{table}[htbp]
\centering
\caption{Comparison of v6 (completed) and v7 (in progress) campaigns.
  Canon~EM is the best canonical exact-match observed so far.}
\label{tab:v7_v6_comparison}
\small
\begin{tabular}{lll}
\toprule
\textbf{Metric} & \textbf{v6 (18\,h)} & \textbf{v7 (15\,h, ongoing)} \\
\midrule
Human interventions     & 7 directives         & 0 \\
Experiments             & 14                   & 4 (deeper, not wider) \\
Novel approach          & None (replicated v5) & Graph inference pipeline (new) \\
Literature search       & None                 & MolSeek-OCR, MolNexTR, MolScribe \\
World model versions    & 18 (abandoned after restart)
                                               & 14 (active, with research plan) \\
\texttt{update\_world\_model()} & Failed (API key) & Working (\texttt{IS\_LOCAL} fix) \\
Best canon~EM           & 0.905                & 0.9032 (and climbing) \\
Primary model           & Claude Opus 4.7      & Kimi K2.6 (first non-Anthropic) \\
Strategic pivots        & Human-directed       & Self-directed \\
\bottomrule
\end{tabular}
\end{table}

The contrast between the two campaigns is instructive.  v6 ran 14
experiments in 18 hours and reproduced the v5 baseline efficiently,
but introduced no new scientific approach.  v7 has run 4 experiments in
15 hours but discovered and built the graph inference pipeline, a
capability that v5 and v6 lacked entirely.  v6 optimized for
throughput; v7 invests in infrastructure and targeted experiments.  The
two strategies are complementary rather than competing, and it is too
early to determine which produces a higher final canon~EM.


\section{Preliminary observations}
\label{sec:v7_observations}

\begin{enumerate}
  \item \textbf{Kimi K2.6 performs well as an autonomous research
    agent.}  Code quality, reasoning depth, and strategic decisions
    are comparable to Claude Opus on this task, at zero API cost
    (self-hosted on the cluster).  The 262K context window has not been
    a constraint so far.

  \item \textbf{The graph inference discovery is a genuine research
    contribution.}  Literature search combined with code inspection in
    the first hour of v7 found what iterative experimentation across
    v5 and v6 did not: the multitask graph heads were trained but
    never used.  This validates the v7 mandatory-literature-search
    rule and suggests that targeted reading is a higher-value activity
    than additional training runs when the problem is diagnostic rather
    than optimization.

  \item \textbf{The working world model produces richer state than
    v6's direct mutations.}  The research plan (r0 through r5) shows
    structured hypothesis-to-experiment mapping.  The 9 established
    findings with confidence levels provide a queryable knowledge base
    that Aries consults before designing new experiments.

  \item \textbf{v7 runs fewer but deeper experiments.}  v6 optimized
    for throughput (14 experiments in 18 hours); v7 builds
    infrastructure first (graph pipeline, evaluation tools, data
    loaders) then runs targeted experiments.  The strategies differ in
    allocation of wall-clock time, and it is not yet clear which
    approach yields higher final accuracy.

  \item \textbf{Zero human intervention is maintained.}  The
    behavioral rules (no sleeping beyond 60\,s, mandatory world model
    update) appear to be followed, though the world model has not been
    updated since v014 (approximately 1 hour into the campaign).
    Whether this represents compliance drift or a natural pause during
    long training runs will become clear as the campaign continues.
\end{enumerate}


\section{Status}
\label{sec:v7_status}

Run~4 (stereo fine-tune from the Run~3 baseline) is training.  If it
exceeds 0.91 canonical exact-match, Aries plans to combine the
stereo-fine-tuned model with the graph inference pipeline.  This
combination, where sequence-decoded SMILES provides the molecular
graph and graph-decoded wedge bonds provide stereochemistry, was never
attempted in v5 or v6.

The campaign is ongoing.  This section will be updated when results
are available.


==> sections/ocsr_markush/datasets_provenance_DRAFT.tex <==
%% ============================================================================
%% DRAFT provenance expansions for sections/ocsr_markush/datasets.tex
%% NOT yet wired into the build. Review against the existing datasets.tex voice
%% and merge the paragraphs into the corresponding subsections by hand.
%%
%% Every number below is verified against an on-cluster manifest or run record;
%% the verifying field/path is named in a trailing % comment. Items that could
%% NOT be verified are flagged with %% UNVERIFIED / %% DISCREPANCY and must be
%% resolved before merge.
%% ============================================================================

%% ----------------------------------------------------------------------------
%% Expansion for \subsection{Training data} -> \paragraph{Markush.}
%% ----------------------------------------------------------------------------

\paragraph{Markush base mixture (250k).}
The Markush base mixture is a deterministic 250{,}000-row SFT mix assembled by
\texttt{scripts/build\_stable\_scaling\_sft\_mix.py} (seed 74) from two prepared
partitions: an 80\% \emph{base} partition (200{,}000 rows) drawn from the prepared
public-plus-molparser canonical pool, and a 20\% \emph{hard-replay} partition
(50{,}000 rows) drawn from a targeted hard-slice replay set
(\texttt{no-synthetic-250k-seed74-80base-20hard/manifest.json}).
% partition_counts: {base:200000, hard:50000}; written_rows 250000; seed 74
Every target is a canonicalized \texttt{cxsmiles\_opt} record
(\texttt{target\_format\_counts}: 250{,}000 rows under
\texttt{"canonicalized cxsmiles\_opt"}); of these, 155{,}415 were already
canonical and 94{,}585 were canonicalized at prep time
(\texttt{target\_canonicalization\_status\_counts}). The 44{,}856 molparser rows
enter via a two-stage target derivation
(\texttt{molparser\_esmiles->cxsmiles\_opt->canonicalized\_cxsmiles\_opt}).
% target_source_counts: cxsmiles_opt->...:205144, molparser_esmiles->...:44856

Across the full mix the row provenance is 152{,}620 MarkushGenerator-1 synthetic
(\texttt{mg1\_synthetic}), 52{,}524 USPTO-derived molecule rows
(\texttt{uspto\_mol\_m}), and 44{,}856 molparser-converted rows
(\texttt{molparser}); by rendering mode this is 152{,}620
\texttt{patent\_image\_markush}, 52{,}524 \texttt{structure\_only\_markush}, and
44{,}856 \texttt{molparser\_converted\_markush}.
% top-level source_counts / mode_counts in the same manifest
The hard-replay partition contributes 35{,}478 \texttt{mg1\_synthetic} and
14{,}522 \texttt{uspto\_mol\_m}; the base partition contributes 117{,}142
\texttt{mg1\_synthetic}, 38{,}002 \texttt{uspto\_mol\_m}, and 44{,}856
\texttt{molparser}.
% per-partition source_counts in the partitions[] array

%% ----------------------------------------------------------------------------
%% Expansion for \subsection{Training data} -> \paragraph{OCSR.}
%% ----------------------------------------------------------------------------

\paragraph{Dedicated OCSR training data.}
The dedicated OCSR model (best checkpoint \texttt{v8-3}, canonical exact match
0.9397) is trained from scratch on four inputs assembled at launch time
(verified from the recorded launch commands under
\texttt{campaigns/ocsr/v10/} and the \texttt{v8-3} run log).
% launch commands: launch_main.sh / direct_launch.sh / run_continue.sh etc.
The molecule sources are taken from the public Hugging Face mirror
\texttt{CYF200127/MolNexTR}.
% notes/research_log.md L39/L41: train_pubchem.csv 1,000,000 rows; train_uspto.zip -> train_uspto.csv 680,220 rows
\begin{description}[leftmargin=1.2em,itemsep=2pt,topsep=2pt]
  \item[PubChem-1M.] \texttt{train\_pubchem.csv}, 1{,}000{,}000 molecules,
  rendered on the fly with the vendored EPAM Indigo renderer
  (\texttt{PubChemIndigoDataset}; \texttt{--pubchem\_csv}).
  \item[USPTO-680k.] \texttt{train\_uspto.csv}, 680{,}220 rows, with images
  pre-rendered from \texttt{train\_uspto.zip} and loaded from disk
  (\texttt{UsptoMolDataset}; \texttt{--uspto\_csv} + \texttt{--uspto\_image\_root}).
  \item[Stereo-enriched curriculum.] \texttt{stereo\_200k\_white/train.csv},
  200{,}000 white-background stereo-rich rows, oversampled $\times 2$
  (\texttt{--stereo\_csv} + \texttt{--stereo\_repeat 2}).
  \item[Canary-similar PubChem.] \texttt{canary\_similar\_pubchem.csv}, 64{,}752
  rows mined for adjacent-ring stereocenters, oversampled $\times 2$
  (\texttt{--extra\_pubchem\_csv} + \texttt{--extra\_pubchem\_repeat 2}).
\end{description}
With the two $\times 2$ oversamples this gives an effective training-set size of
2{,}209{,}724 rows
($1{,}000{,}000 + 680{,}220 + 2\times200{,}000 + 2\times64{,}752$).
% dataset_size=2209724 in v8-3 train.log and notes/experiments/v8-2-analysis.json
Targets are RDKit-canonical SMILES (\texttt{target\_format=chartok\_smiles\_only}).
The encoder is a Swin-B/384 ImageNet backbone with a six-layer transformer
decoder (\texttt{checkpoints/v8-3-recipe.json}; \texttt{notes.primary\_recipe =
MolNexTR}, ImageNet backbone allowed, OCSR-specific pretrained checkpoints
forbidden).

%% DISCREPANCY (must reconcile before merge): the task brief described the OCSR
%% inputs as "stereo-curriculum (50,336, oversampled x20)" and "canary RDKit
%% (50,336)", assembled by "prepare_data.py". The on-cluster v8-3 launch
%% commands and the recorded dataset_size=2,209,724 instead show
%% stereo_200k_white (200,000, x2) + canary_similar_pubchem (64,752, x2), and
%% the launch is plain `python -m autoresearch.train ...` (no prepare_data.py
%% was found on disk; the rendered data was discarded and is regenerated by the
%% pipeline). The 50,336-row files DO exist on disk
%% (datasets-curated/v6-fresh/stereo_curriculum_v2.csv and
%% canary_rdkit_training.csv, both 50,336 lines incl. header), and the "x20
%% oversampling of 50k stereo-rich molecules" appears verbatim in
%% notes/v7_summary.json as a description of an EARLIER iteration (v7 "Scratch
%% stereo enriched"), NOT the headline v8-3 run. I have written the VERIFIED
%% v8-3 composition above. Confirm which recipe the paper intends to report.

%% Higher-level summary line for \paragraph{OCSR.} prose (replaces the existing
%% "about 1.68 million unique molecule images ... roughly 2.21 million effective
%% training rows" sentence, which is consistent with the verified counts):
%%   1,000,000 (PubChem) + 680,220 (USPTO) = 1,680,220 unique molecule images;
%%   2,209,724 effective rows after the two x2 oversamples.

%% ----------------------------------------------------------------------------
%% Expansion for \subsection{Joint training data} (OCSR-as-Markush mixes)
%% ----------------------------------------------------------------------------

\paragraph{OCSR-as-Markush mixes and decontamination.}
The joint model adds an ordinary-molecule mixture by converting OCSR rows into
the no-variable-group Markush special case. The mixes are prepared at three
target ordinary-molecule fractions; the count at fraction $f$ over a fixed
250{,}000-row Markush base is
$\mathrm{round}\!\left(\tfrac{f}{1-f}\times 250000\right)$, giving 13{,}158
(5\%), 27{,}778 (10\%), and 44{,}118 (15\%) ordinary rows for total mix sizes of
263{,}158, 277{,}778, and 294{,}118.
% target_ocsr_count_formula, ocsr_count, total_rows in
% ocsr-fraction-{5,10,15}pct-seed74-decontam/manifest.json
The ordinary rows are drawn from the MolScribe OCSR pool
(\texttt{molscribe-ocsr/.../unified.jsonl}, 680{,}220 source rows; 625{,}089
trainable rows survive validity and eligibility filtering) and encoded in the
unified format with an empty extension,
\verb|<markush><cxsmi>SMILES</cxsmi><stable></stable></markush>|
(\texttt{ocsr\_row\_as\_no\_extension\_markush} in
\texttt{prepare\_final\_multitask\_sft.py}).
% decontamination.source_rows 680220, trainable_kept_rows 680140,
% eligible_decontaminated_rows 625089

Before conversion the pool is decontaminated against the four ordinary-molecule
OCSR evaluation sets (CLEF, JPO, UOB, USPTO). Eligibility is decided by
RDKit-canonical SMILES match: any pool molecule whose canonical SMILES collides
with an evaluation molecule is removed. The evaluation reference set is 12{,}870
rows / 11{,}259 unique canonical SMILES, and 80 overlapping pool molecules are
removed in every fraction (\texttt{decontamination\_removed\_count} = 80). A
post-decontamination check then re-scans the materialized mix and finds zero
remaining overlap in all three fractions
(\texttt{post\_decontamination\_leakage\_check.overlap\_rows} = 0,
\texttt{severity} = \texttt{none}).
% ocsr_eval_canonical_smiles.rows 12870, unique_canonical_smiles 11259;
% decontamination_removed_count 80; post_decontamination_leakage_check.overlap_rows 0
% cross-checked in ocsr-fraction-decontam-summary-seed74.json (all three: 0)

%% NOTE: the existing datasets.tex headline 5%% mixture cites "about 13,158
%% no-variable-group records" and "about 5,373 of 16,667 USPTO rows" filtered.
%% The 13,158 here is the DECONTAMINATED MolScribe-pool mix (fraction formula
%% above), which is verified. The 16,667/5,373 placeholder-filter numbers live
%% in the existing appendix (\app:additional, "No-extension placeholder
%% filtering") and were NOT re-verified in this pass -- they are a different
%% (USPTO ordinary-row) pool. Flag if a single consistent number is wanted.

%% ----------------------------------------------------------------------------
%% Expansion for \subsection{Joint training data} (synthetic-mix arm)
%% Replaces / extends the "explored but not promoted" sentence -- see CAVEAT.
%% ----------------------------------------------------------------------------

\paragraph{Synthetic Markush-rendering mixture (under re-test).}
A synthetic Markush arm augments the 250{,}000-row base with eval-aligned
synthetic rows. The synthetic pool is generated by sampling a PubChem-scaffold
pool, decorating it with the \texttt{eval\_aligned} profile in
\texttt{markush.data.pipeline}, and rendering with MarkushGenerator in
train-like, structure-only mode. Two pools are mixed in:
\texttt{existing-eval-like-10k} (10{,}000 rows) and
\texttt{existing-eval-like-100k} (100{,}000 rows), producing mixes of 260{,}000
and 350{,}000 rows respectively.
% synthetic-mix-{260k,350k}-seed74/manifest.json: written_rows 260000 / 350000;
% synth partition selected_count 10000 / 100000
The synthetic share is the 10{,}000-row pool at $\approx$3.8\% of the 260k mix
and the 100{,}000-row pool at $\approx$28.6\% of the 350k mix.
% 10000/260000 = 3.8%; 100000/350000 = 28.6%
Both synthetic pools were checked for evaluation leakage against the full
1{,}055-row public Markush evaluation set (IP5-M $+$ M2S $+$ USPTO-Markush) by
canonical-structure match and showed zero overlap
(\texttt{synthetic-mix-leakage-check-seed74.json}: \texttt{eval\_rows} 1{,}055,
both pools \texttt{overlap\_rows} 0, \texttt{severity} \texttt{none}); the 100k
pool deduplicates to 60{,}388 unique rows
(\texttt{eligible\_rows} in the 350k manifest).
% leakage-check: eval_rows 1055, pool overlap_rows 0/0; 350k synth eligible_rows 60388

\emph{Status caveat.} An earlier campaign reported the synthetic arm as
explored-but-not-promoted (the renderer-fidelity and seed-coverage findings in
Appendix~\ref{app:additional}). The mixes documented here are the current
synthetic-mix ablation arms and are being re-tested; we do not assert a final
promote/no-promote outcome for them in this draft.
%% CAVEAT: do NOT state an outcome for the synthetic arm here. The existing
%% datasets.tex says "explored but not promoted"; the present arms are a
%% re-test. Resolve the narrative once the ablation result lands.


==> sections/system_design.tex <==
\section{System Design}
\label{sec:system}

\subsection{The AutoResearch Loop for Science}

Our system follows the three-file pattern established by Karpathy, adapted for scientific investigation:

\begin{itemize}[nosep]
  \item \texttt{experiment.py} --- the agent's sandbox. Initially contains a baseline MolScribe OCSR pipeline. The agent modifies this file each iteration.
  \item \texttt{evaluate.py} --- immutable evaluator computing four metrics: 1$-$exact\_match\_rate (primary, lower is better), validity\_rate, mean Tanimoto similarity, and stereo accuracy. Stratified reporting by molecular tags.
  \item \texttt{program.md} --- research strategy document with six phases (model selection $\rightarrow$ pre-processing $\rightarrow$ post-processing $\rightarrow$ ensembles $\rightarrow$ fine-tuning $\rightarrow$ RL), domain knowledge, and constraints.
\end{itemize}

The agent follows the prescribed loop on the development benchmark: modify \texttt{experiment.py}, run it to produce \texttt{results.json}, then run \texttt{evaluate.py -p results.json} to score. The evaluator was verified unchanged throughout the study (MD5 \texttt{28e9b1...e1d3}, matching on both source and cluster). For real-benchmark evaluation, the agent ran models directly on HuggingFace benchmark images and computed exact-match using the same canonicalization logic as \texttt{evaluate.py}, since the real benchmarks (12,901 images) are not part of the development manifest.

\paragraph{Beyond the prescribed loop.} The three-file pattern served as the starting structure, but Aries organically expanded beyond it as the research progressed. Once the 20-image development benchmark saturated at 20/20 (Iteration~5), the agent autonomously built parallel evaluation infrastructure to scale to the four real benchmarks (12,901 images total). This included custom runner scripts for MolSight inference on HuggingFace datasets (\texttt{run\_molsight\_real.py}), a 16-worker multiprocessed synthetic data generator (\texttt{build\_synth\_data.py}), and a LoRA training script with its own evaluation loop (\texttt{jpo\_lora\_train.py}). All real-benchmark evaluation used the same SMILES canonicalization logic as \texttt{evaluate.py}, but operated on datasets outside the development manifest. The prescribed loop remained the formal checkpoint---every \texttt{experiment.py} modification was validated against \texttt{evaluate.py} on the development set---but the agent's actual research process grew substantially beyond it. This evolution from following a prescribed protocol to building custom research infrastructure is itself an interesting behavioral observation: the agent recognized when the prescribed evaluation was insufficient and adapted.

\subsection{The Agent}
\label{sec:agent}

Aries, the next iteration of Edison Scientific's Kosmos agent~\citep{mitchener2025kosmos}, operates inside a GPU-enabled sandbox on a Slurm-managed cluster. Available tools include: Python execution via Jupyter (\texttt{run\_cell}), file editing, web search, sub-agent dispatch for literature queries and data retrieval, and access to the e14c library for data storage and task management.

The hardware environment consists of 8$\times$ NVIDIA H100 80GB HBM3 GPUs, 104 CPUs, and shared NFS storage across 32 worker nodes. All experiments use a single node.

\subsection{Orchestration}

When directed, Aries operates in \textbf{autonomous mode}---planning, executing, and evaluating experiments without waiting for human approval between iterations. Communication occurs via an HTTP API, where messages are queued per-session. In this study, the human operator sent 5 directive messages over the course of the run; the agent generated 700+ messages including 300+ executed code cells.

